Improved Neural Radiance Fields Using Pseudo-depth and Fusion

Since the advent of Neural Radiance Fields, novel view synthesis has received tremendous attention. The existing approach for the generalization of radiance field reconstruction primarily constructs an encoding volume from nearby source images as additional inputs. However, these approaches cannot efficiently encode the geometric information of real scenes with various scale objects/structures. In this work, we propose constructing multi-scale encoding volumes and providing multi-scale geometry information to NeRF models. To make the constructed volumes as close as possible to the surfaces of objects in the scene and the rendered depth more accurate, we propose to perform depth prediction and radiance field reconstruction simultaneously. The predicted depth map will be used to supervise the rendered depth, narrow the depth range, and guide points sampling. Finally, the geometric information contained in point volume features may be inaccurate due to occlusion, lighting, etc. To this end, we propose enhancing the point volume feature from depth-guided neighbor feature fusion. Experiments demonstrate the superior performance of our method in both novel view synthesis and dense geometry modeling without per-scene optimization.

==> srcs/tables/4-2_res-syn-color.tex <==
\begin{tabular}{
m{2.0cm}
m{1.5cm}<{\centering}m{1.5cm}<{\centering}m{1.5cm}<{\centering}
}
    \toprule
    Methods & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
    PixelNeRF~\cite{yu2021pixelnerf} & - & - & - \\
    IBRNet~\cite{wang2021ibrnet}     & - & - & - \\
    MVSNeRF~\cite{chen2021mvsnerf}   & - & - & - \\
    ENeRF                            & 26.65 & 0.947 & 0.072 \\
    Ours                             & - & - & - \\
    \bottomrule
\end{tabular}

==> srcs/tables/4-ablation-scale.tex <==
\begin{tabular}{
m{3.2cm}
m{1.15cm}<{\centering}m{1.1cm}<{\centering}m{1.2cm}<{\centering}
}
\toprule
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
Only use $3^{th}$ stage & 25.27 & 0.912 & 0.192 \\
All stages no fusion & 26.28 & 0.934 & 0.162 \\
All stages AVG fusion & 26.84 & 0.938 & 0.157 \\
All stages GRU fusion & \textbf{27.32} & \textbf{0.942} & \textbf{0.150} \\
\bottomrule
\end{tabular}

==> srcs/tables/4-res_dtu_color.tex <==
\begin{tabular}{
m{2.4cm}
m{1.3cm}<{\centering}m{1.3cm}<{\centering}m{1.45cm}<{\centering}
}
\toprule
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
PixelNeRF\cite{yu2021pixelnerf} & 19.13 & 0.789 & 0.382 \\
IBRNet\cite{wang2021ibrnet} & 26.04 & 0.917 & 0.190 \\
MVSNeRF\cite{chen2021mvsnerf} & 26.63 & 0.931 & 0.168 \\
DS-NeRF\cite{deng2022depth} & 16.90 & 0.570 & 0.450 \\
Point-NeRF\cite{xu2022point} & 23.89 & 0.874 & 0.203 \\
% NeuRay & - & - & - \\
\midrule
Ours & \textbf{27.84} & \textbf{0.946} & \textbf{0.141} \\
\bottomrule
\end{tabular}

==> srcs/tables/4-res_dtu_depth.tex <==
\begin{tabular}{
m{2.4cm}
m{1.3cm}<{\centering}m{1.3cm}<{\centering}m{1.45cm}<{\centering}
}
\toprule
Method & Abs err $\downarrow$ & $<$0.05 $\uparrow$ & In range $\uparrow$ \\
\midrule
Stage 1 & 0.022  & 0.918  & \textbf{1.000}  \\
Stage 2 &  0.016 & 0.941 & 0.995  \\
Stage 3 &  \textbf{0.015} & \textbf{0.943} & 0.946  \\
\midrule
PixelNeRF\cite{yu2021pixelnerf} & 0.239  & 0.187 & -  \\
MVSNeRF\cite{chen2021mvsnerf} & 0.035 & 0.866 & - \\
% NeuRay &  &  &  \\
Ours & \textbf{0.031} & \textbf{0.906} & - \\
\bottomrule
\end{tabular}

==> srcs/tables/4-res_others.tex <==
% \begin{tabular}{
% m{2.0cm}
% m{1.5cm}<{\centering}m{1.5cm}<{\centering}m{1.5cm}<{\centering}
% }
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{3}{c}{Forward-Facing\cite{mildenhall2019local}/Synthetic Data\cite{mildenhall2021nerf}} \\
% \cmidrule{2-4}
% & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
% \midrule
% PixelNeRF\cite{yu2021pixelnerf} & 11.24/7.39 & 0.486/0.658 & 0.671/0.411 \\
% IBRNet\cite{wang2021ibrnet} & 21.79/22.44 & 0.786/0.874 & 0.279/0.195 \\
% MVSNeRF\cite{chen2021mvsnerf} & 21.93/23.62 & 0.795/0.897 & 0.252/0.176 \\
% Ours & -/\textbf{24.53} & -/\textbf{0.931} & -/\textbf{0.105} \\
% \bottomrule
% \end{tabular}


\begin{tabular}{
m{2.0cm}
m{1.5cm}<{\centering}m{1.5cm}<{\centering}m{1.5cm}<{\centering}
}
\toprule
Methods & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
PixelNeRF\cite{yu2021pixelnerf} & 7.39 & 0.658 & 0.411 \\
IBRNet\cite{wang2021ibrnet} & 22.44 & 0.874 & 0.195 \\
MVSNeRF\cite{chen2021mvsnerf} & 23.62 & 0.897 & 0.176 \\
Ours & \textbf{24.53} & \textbf{0.931} & \textbf{0.105} \\
\bottomrule
\end{tabular}

==> srcs/tables/sup_1.tex <==
\begin{tabular}{
p{1.5cm}
p{0.9cm}<{\centering}p{0.9cm}<{\centering}p{0.9cm}<{\centering}
p{0.9cm}<{\centering}p{0.9cm}<{\centering}
}
    \toprule
    Scan & \#1 & \#8 & \#21 & \#103 & \#114 \\
    \midrule
    \multicolumn{6}{c}{PSNR $\uparrow$} \\
    \midrule
    PixelNeRF  & 21.64 & 23.70 & 16.04 & 16.76 & 18.40 \\
    IBRNet & 25.97 & 27.45 & 20.94 & 27.91 & 27.91 \\
    MVSNeRF & 26.96 & 27.43 & 21.55 & 29.25 & 27.99 \\
    ENeRF & 28.85 & 29.05 & 22.53 & 30.51 & 28.86 \\
    Ours  & 29.44 & 30.04 & 22.02 & 31.32 & 29.78 \\
    \midrule
    \multicolumn{6}{c}{SSIM $\uparrow$} \\
    \midrule
    PixelNeRF & 0.827 & 0.829 & 0.691 & 0.836 & 0.763\\
    IBRNet & 0.918 & 0.903 & 0.873 & 0.950 & 0.943\\
    MVSNeRF & 0.937 & 0.922 & 0.890 & 0.962 & 0.949\\
    ENeRF & 0.958 & 0.955 & 0.916 & 0.968 & 0.961\\
    Ours  & 0.961 & 0.951 & 0.914 & 0.970 & 0.961\\
    \midrule
    \multicolumn{6}{c}{LPIPS $\downarrow$} \\
    \midrule
    PixelNeRF & 0.373 & 0.384 & 0.407 & 0.376 & 0.372 \\
    IBRNet & 0.190 & 0.252 & 0.179 & 0.195 & 0.136 \\
    MVSNeRF & 0.155 & 0.220 & 0.166 & 0.165 & 0.135 \\
    ENeRF & 0.086 & 0.119 & 0.107 & 0.107 & 0.076 \\
    Ours  & 0.091 & 0.071 & 0.176 & 0.120 & 0.021 \\
    \bottomrule

\end{tabular}

==> srcs/tables/sup_2.tex <==
\begin{tabular}{
p{1.5cm}
p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}
p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}
}
    \toprule
    Scan & Chair & Drums & Ficus & Hotdog & Lego & Materials & Mic & Ship \\
    \midrule
    \multicolumn{9}{c}{PSNR $\uparrow$} \\
    \midrule
    PixelNeRF & 7.18 & 8.15 & 6.61 & 6.80 & 7.74 & 7.61 & 7.71 & 7.30\\
    IBRNet & 24.20 & 18.63 & 21.59 & 27.70 & 22.01 & 20.91 & 22.10 & 22.36\\
    MVSNeRF & 23.35 & 20.71 & 21.98 & 28.44 & 23.18 & 20.05 & 22.62 & 23.35\\
    ENeRF & 24.49 & 19.03 & 21.26 & 30.62 & 21.89 & 21.47 & 23.38 & 23.90\\
    Ours  & 23.90 & 20.13 & 20.55 & 32.81 & 21.82 & 25.99 & 28.73 & 25.05 \\
    \midrule
    \multicolumn{9}{c}{SSIM $\uparrow$} \\
    \midrule
    PixelNeRF & 0.624 & 0.670 & 0.669 & 0.669 & 0.671 & 0.644 & 0.729 & 0.584\\
    IBRNet & 0.888 & 0.836 & 0.881 & 0.923 & 0.874 & 0.872 & 0.927 & 0.794\\
    MVSNeRF & 0.876 & 0.886 & 0.898 & 0.962 & 0.902 & 0.893 & 0.923 & 0.886\\
    ENeRF & 0.912 & 0.855 & 0.881 & 0.959 & 0.892 & 0.889 & 0.937 & 0.822\\
    Ours  & 0.099 & 0.188 & 0.129 & 0.115 & 0.180 & 0.128 & 0.081 & 0.303 \\
    \midrule
    \multicolumn{9}{c}{LPIPS $\downarrow$} \\
    \midrule
    PixelNeRF & 0.386 & 0.421 & 0.335 & 0.433 & 0.427 & 0.432 & 0.329 & 0.526\\
    IBRNet & 0.144 & 0.241 & 0.159 & 0.175 & 0.202 & 0.164 & 0.103 & 0.369\\
    MVSNeRF & 0.282 & 0.187 & 0.211 & 0.173 & 0.204 & 0.216 & 0.177 & 0.244\\
    ENeRF & 0.043 & 0.056 & 0.072 & 0.039 & 0.075 & 0.073 & 0.040 & 0.181\\
    Ours  & 0.071 & 0.154 & 0.122 & 0.061 & 0.116 & 0.107 & 0.053 & 0.198 \\
    \bottomrule

\end{tabular}

==> srcs/tables/sup_3.tex <==
\begin{tabular}{
p{1.5cm}
p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}
p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}
}
    \toprule
    Scan & Fern & Flower & Fortress & Horns & Leaves & Orchids & Room & Trex \\
    \midrule
    \multicolumn{9}{c}{PSNR $\uparrow$} \\
    \midrule
    PixelNeRF & 12.40 & 10.00 & 14.07 & 11.07 & 9.85 & 9.62 & 11.75 & 10.55 \\
    IBRNet & 20.83 & 22.38 & 27.67 & 22.06 & 18.75 & 15.29 & 27.26 & 20.06 \\
    MVSNeRF & 21.15 & 24.74 & 26.03 & 23.57 & 17.51 & 17.85 & 26.95 & 23.20 \\
    ENeRF & 20.88 & 24.78 & 28.63 & 23.51 & 17.78 & 17.34 & 28.94 & 20.37 \\
    Ours  & 20.91 & 24.15 & 28.28 & 24.20 & 18.43 & 16.07 & 29.66 & 20.54 \\
    \midrule
    \multicolumn{9}{c}{SSIM $\uparrow$} \\
    \midrule
    PixelNeRF & 0.531 & 0.433 & 0.674 & 0.516 & 0.268 & 0.317 & 0.691 & 0.458 \\
    IBRNet & 0.710 & 0.854 & 0.894 & 0.840 & 0.705 & 0.571 & 0.950 & 0.768 \\
    MVSNeRF & 0.638 & 0.888 & 0.872 & 0.868 & 0.667 & 0.657 & 0.951 & 0.868 \\
    ENeRF & 0.727 & 0.890 & 0.920 & 0.866 & 0.685 & 0.637 & 0.958 & 0.778 \\
    Ours & 0.701 & 0.871 & 0.893 & 0.814 & 0.709 & 0.579 & 0.969 & 0.721 \\
    \midrule
    \multicolumn{9}{c}{LPIPS $\downarrow$} \\
    \midrule
    PixelNeRF & 0.650 & 0.708 & 0.608 & 0.705 & 0.695 & 0.721 & 0.611 & 0.667 \\
    IBRNet & 0.349 & 0.224 & 0.196 & 0.285 & 0.292 & 0.413 & 0.161 & 0.314 \\
    MVSNeRF & 0.238 & 0.196 & 0.208 & 0.237 & 0.313 & 0.274 & 0.172 & 0.184 \\
    ENeRF & 0.235 & 0.168 & 0.118 & 0.200 & 0.245 & 0.308 & 0.141 & 0.259 \\
    Ours  & 0.296 & 0.198 & 0.185 & 0.243 & 0.243 & 0.395 & 0.104 & 0.281\\
    \bottomrule

\end{tabular}
